Regret-Minimizing Contracts: Agency Under Uncertainty

We study the fundamental problem of designing contracts in principal-agent problems under uncertainty. Previous works mostly addressed Bayesian settings in which principal's uncertainty is modeled as a probability distribution over agent's types. In this paper, we study a setting in which the principal has no distributional information about agent's type. In particular, in our setting, the principal only knows some uncertainty set defining possible agent's action costs. Thus, the principal takes a robust (adversarial) approach by trying to design contracts which minimize the (additive) regret: the maximum difference between what the principal could have obtained had them known agent's costs and what they actually get under the selected contract.

==> src/FPTAS.tex <==









==> src/Hardness.tex <==



==> src/PTAS.tex <==





==> src/deltaBound.tex <==



==> src/existence_2.tex <==













==> src/prelim.tex <==












 

==> src/prelim2.tex <==


\section{ Prelim}

Let $\cC\subset[0,1]^{|A|}$ a convex set.

Every $\vc\in\cC$ defines a cost vector $\vc[a]:=c_a$ for the costly action of the agent.
Interaction as follow:

\begin{enumerate}
	\item The principal commits to a menu of randomize contracts $\Gamma$ of size $D$. Where $\gamma_i\in\Delta(\mathbb{R}^m)$ for $i\in[D]$ is a randomized contract \ie a distribution over possible payments vector
	\item The agent picks a randomized contract $\gamma\in\Gamma$
	\item The principal samples a contract $\vp\sim\gamma$ and commits to it
	\item The agent performs an action $a$ (BR) to $\vp$ which costs $c_a$
	\item An outcome $\omega\in\Omega$ is sampled accordingly to a outcome distribution $F_a$
	\item Utility $u(\omega)$ is returned to the principal which pays the agent $p(\omega)$
\end{enumerate}

Set of deterministic contracts: $\determ\equiv\reals^m_{\ge 0}$ 

Let $U(\Gamma,\vc)$ the expected utility of the principal that commits to a menu of randomized contract $\Gamma$ against an agent with cost vector $\vc\in\cC$.

\begin{lemma}
	For every $\vc\in\cC$ there exists a deterministic contract $\vp\in\reals^m_{\ge 0}$ which is optimal.
	\[
	\OPT(\vc)=\sup\limits_{\vp\in\determ}U(\vp, \vc)
	\]
\end{lemma}

\begin{definition}
	\[
	\diam(\cC)\defeq\sup\limits_{\vc,\vc'\in\cC}\|\vc-\vc'\|_{\infty}.
	\]
\end{definition}

\begin{theorem}\label{th:deltaopt}
For every $\vc\in\cC$ there exists a deterministic contract $\vp'$ such that
\[
U(\vp',\tilde\vc)\ge \OPT(\vc)-2\sqrt{2\diam(\cC)},\, \forall \tilde\vc\in\cC.
\]
\end{theorem}

\begin{proof}
	Call $\vp^\star$ the optimal contract for the cost vector $\vc$. Thus:
	\[
	\OPT(\vc) = U(\vp^\star, \vc).
	\]
	Take any $\tilde \vc\in\cC$. Then, by definition of diameter of $\cC$, we have $|\tilde c_a-c_a|\le \diam(\cC)$.
	
	First observe that the contract $\vp^\star$ is a $2\diam(\cC)$-IC contract for the cost vector $\tilde\vc$.
	Formally, let $a$ the best response for the cost vector $\vc$, then $a$ is a $2\delta$ besr response for contract $\vp^\star$ against the cost vector $\tilde\vc$.
	For all $a'\in A$ the following holds:
	\begin{align}
		\E_{\omega\sim F_a}[p^\star_\omega]-\tilde c_a&\ge\E_{\omega\sim F_a}[p^\star_\omega]- c_a - \diam(\cC)\nonumber\\
		&\ge \E_{\omega\sim F_{a'}}[p^\star_\omega]- c_{a'} - \diam(\cC)\nonumber\\
		&\ge \E_{\omega\sim F_{a'}}[p^\star_\omega]-\tilde c_{a'} - 2\diam(\cC)\label{eq:deltabr}.
	\end{align}
	which proves that $a$ is still a $2\diam(\cC)$ best response to $\vp^\star$.
	
	Now design a new contract $\vp'$ which add a small fraction $\alpha$ of the principal utility to the agent.
	Formally:
%
	\begin{align}
		p_\omega'&:=p_\omega^\star+\alpha (u(\omega)-p^\star_\omega)\\
		&=(1-\alpha) p_\omega^\star+\alpha u(\omega)
	\end{align}	
	
	If the agent plays an action $a'\in A$ the utility of the agent under contract $\vp'$ is $(1-\alpha)$ the utility under contract $\vp^\star$.
	\begin{equation}\label{eq:scalingutils}
	\E_{\omega\sim F_{a}}[u(\omega)-p'_\omega]=(1-\alpha)	\E_{\omega\sim F_{a}}[u(\omega)-p^\star_\omega]
	\end{equation}
%	In particular if $a''=a$ (BR does not change between contract $\vp'$ and $\vp^\star$) then this implies that
%	\[
%	U(\vp',\tilde\vc) = (1-\alpha) U(\vp^\star, \vc) = (1-\alpha)\OPT(\vc)\ge\OPT(\vc)-\alpha.
%	\]
	%
	Assume now that the best response to contract $\vp'$ is $a''$. Then
	\begin{align*}
		\E_{\omega\sim F_{a^{''}}}[p'_\omega]-\tilde c_{a''}&=(1-\alpha)\E_{\omega\sim F_{a^{''}}}[p^\star_\omega]+\alpha\E_{\omega\sim F_{a''}}[u(\omega)]-\tilde c_{a''}\tag{Definition of $\vp'$}\\
		&\ge(1-\alpha) \E_{\omega\sim F_a}[p_\omega^\star]+\alpha \E_{\omega\sim F_a}[u(\omega)]-\tilde c_a\tag{$a''$ is BR to $vp'$}\\
		&=\E_{\omega\sim F_a}[p_\omega^\star]-\tilde c_a+\alpha\left(\E_{\omega\sim F_a}[u(\omega)-p_\omega^\star]\right)\\
		&\ge \E_{\omega\sim F_{a''}}[p_\omega^\star]-\tilde c_{a''}+\alpha \OPT(\vc)-2\diam(\cC)\tag{\Cref{eq:deltabr}}\\
	\end{align*}
%
	Rearranging we obtain:
	\[
	(1-\alpha)\E_{\omega\sim F_{a^{''}}}[p^\star_\omega]+\alpha\E_{\omega\sim F_{a''}}[u(\omega)]-\tilde c_{a''}\ge \E_{\omega\sim F_{a''}}[p_\omega^\star]-\tilde c_{a''}+\alpha \OPT(\vc)-2\diam(\cC)
	\]
	which simplifies to:
	\[
	\E_{\omega\sim F_{a''}}[u(\omega)-p^\star_\omega]\ge \OPT(\vc)-\frac{2\diam(\cC)}{\alpha}
	\]
	By using \Cref{eq:scalingutils} we get that:
	\[
	U(\vp',\tilde \vc)=\E_{\omega\sim F_{a''}}[u(\omega)-p'_\omega]\ge (1-\alpha)\left(\OPT(\vc)-\frac{2\diam(\cC)}{\alpha}\right)\ge \OPT(\vc)-\left(\frac{2\diam(\cC)}{\alpha}+\alpha\right).
	\]
	Then to minimize the error we take $\alpha=\sqrt{2\diam(\cC)}$ which gives an error of $2\sqrt{2\diam(\cC)}$.
\end{proof}

\begin{corollary}
	For all $\vc,\tilde\vc\in\cC$:
	\[
	|\OPT(\vc)-\OPT(\tilde\vc)|\le \sqrt{\diam(\cC)}
	\]
\end{corollary}
\begin{proof}
	Thanks to \Cref{th:deltaopt}: for every $\vc\in\cC$ there exists a deterministic contract $\vp'$ such that
	\[
	U(\vp',\tilde\vc)\ge \OPT(\vc)-2\sqrt{2\diam(\cC)},\, \forall \tilde\vc\in\cC.
	\]
	but $\OPT(\tilde\vc)\ge U(\vp',\tilde\vc)$ and thus:
	\[
	\OPT(\tilde\vc)\ge\OPT(\vc)-2\sqrt{2\diam(\cC)},\, \forall \tilde\vc\in\cC.
	\]
\end{proof}

The sensitivity of a contract $\vp$ is defined as:
\[
\reg(\vp) = \sup\limits_{\vc\in\cC}\left[\OPT(\vc)-U(\vp,\vc)\right]
\]

\begin{corollary}
	\[
	\inf\limits_{\vp\in\determ}\reg(\vp) \le\sqrt{\diam(\cC)}
	\]
\end{corollary}

\subsection{Existence of robust contracts}

Here we study the existence of the $\inf$ of the following problem:
%
\[
\inf\limits_{p\in\Pi}\reg (\vp).
\]

%\begin{lemma}
%	For all $\vp$ there exists:
%	\[
%	\vc^\star(\vp)\in\arg\max\limits_{c\in\cC}\left[\OPT(\vc)-U(\vp,\vc)\right]
%	\]
%\end{lemma}

%\begin{lemma}
%	For all $\vc$, the function
%	\[
%	\vp\mapsto \OPT(\vc)-U(\vp, \vc)
%	\]
%	is LSC.
%\end{lemma}


\begin{theorem}
	We have that there exists $\vp^\star\in \Pi$ such that
	\[
	\reg(\vp^\star)=\inf\limits_{\vp\in\Pi} \reg(\vp).
	\]
\end{theorem}

\begin{proof}
	Consider the function:
	\[
	g(\vp, \vc):=\OPT(\vc)-U(\vp,\vc)
	\]
	For every $\vc$ the function $\vp\mapsto g(\vp,\vc)$ is LSC. Indeed the first term is independent on $\vp$ and for every $\vc$ the functiion $\vp\mapsto U(\vp,\vc)$ is USC as the ties are broken in favor of the principal (see for \eg \citep{dutting2019simple}).
	
	Then the following claim proves
	\begin{claim}
		If for all $\vc\in\cC$, the function $\vp\mapsto g(\vp,\vc)$ is LSC then the function $\vp\mapsto\sup_{\vc\in\cC}g(\vp,\vc)$ is also LSC.
	\end{claim}
	\begin{proof}
		
	\end{proof}
	Then we have that $\vp\mapsto\reg(\vp)$ is LSC. This would entails the existence of a minima if the $\inf$ would have been on a compact set. However $\Pi$ is not compact. However it is easy to show that the space over which resides the optimum is bounded.
	
	$U(\vzero,\vc)=0$
	\ma{tbc!}
	Consider a contract $\vp$ and assume there exists an outcome $\tilde\omega$ such that $p_{\tilde\omega}\ge\alpha$, then for all $a$:
	\[
	\E_{\omega\sim F_a}[u(\omega)-p_\omega]\le 1-\alpha\eta
	\]
	where $\eta:=\min_{\omega}\max_a F_{a,\omega}$. Thus when $\alpha>1/\eta$ the contract $\vp$ is dominated by the contract $\vzero$, and thus any optimal contract is such that $\|\vp\|_{\infty}\le{1}/{\eta}$.
	
\end{proof}


\begin{theorem}
	The inner $\inf$ might not exists, even for randomized contract.\ma{add figure}
\end{theorem}
\begin{proof}
	Consider the following instance. The agent has two actions $A=\{\varnothing, a\}$, where $\varnothing$ represent the \emph{do nothing} action and $a$ represent the favorable action for the principal. 
	The set of uncertain costs is $\cC=\{c_{\varnothing}=0, c_{a}\in[0,1]\}$.
	Two outcomes $\Omega=\{\omega_{\varnothing}, \omega_{a}\}$ and $F_{\varnothing, \omega_\varnothing}=1$, $F_{\varnothing, \omega_a}=0$, $F_{a, \omega_a}=1$ and $F_{a, \omega_\varnothing}=0$, which means that action $a$ only can result in outcome $\omega_a$ and similarly for $\varnothing$. Then $u_\varnothing=0$ and $u_{a}=1$.
	Consider now a simple randomized contract $\gvec$ that puts probability mass $\gamma(\vp_2)=\gamma(\vp_1)=1/2$ on a contract $\vp_1=(0,1/4)$ and $\vp_2=(0, 3/4)$.
	In this instance the function:
	\begin{align}
	\OPT(\vc)-U(\gvec, \vc)&=1-c_{a}-\sum\limits_{i\in\{1,2\}:p_{i,a}\ge c_{a}}\gvec(\vp_i) (1-p_{i,a})\\
	&=1-c_{a}-\frac{1}{2}\sum\limits_{i\in\{1,2\}:p_{i,a}\ge c_{a}} (1-p_{i,a})\\
	&=1/2-c_a+\begin{cases}
		0&\text{if }c_{a}\in[0,1/4] \\
		3/8&\text{if }c_{a}\in(1/4,3/4]\\
		1/2&\text{if }c_{a}\in(3/4,1]\\
	\end{cases}
	\end{align}
	which is lower-semi continuous and thus does not admit a maximum.
	First note that $\OPT(\vc)-U(\gamma,\vc)<5/8$ for all $\vc=(0,c_a)\in\cC$. Then consider $\vc_\epsilon=(0,1/4+\epsilon)$. We have that:
	\[
	\OPT(\vc_\epsilon)-U(\gvec, \vc_\epsilon) = 5/8-\epsilon
	\]
	for all $\epsilon>0$ which proves that:
	$\sup\limits_{\vc\in\cC}[\OPT(\vc)-U(\gvec, \vc)] = 5/8.$
	On the other hand $\lim_{\epsilon\to 0^+}\OPT(\vc_\epsilon)-U(\gvec, \vc_\epsilon)=1/4$.
\end{proof}

\begin{theorem}
	Let $\cP^R$ the set of randomized contract with finite support. Then the problem
	\[
	\inf\limits_{\gvec\in\cP^R}\reg(\gvec)
	\]
	does not admit a minimum.
\end{theorem}
\begin{proof}
	We will divide the proof into 2 different parts. 1) Construct a family of randomized contract $\gvec_k$ such that they all get at least $\Theta(1/e-1/k)$. 2) Prove that for all $\gvec$ with finite support we have that they get strictly more $1/e$. Thus the inf is not obtained.
	
	\xhdr{Part 1}
	We will construct a sequence of randomized contracts $\gvec_k$ of finite support $k$ and show that they obtain diminishing utility.
	Consider the same instance of above.
	
	For all $k\in\mathbb{N}$, consider the distribution  randomized contracts $\gvec_k$ with support on contracts $\vp^k_1,\ldots, \vp_k^k$ where:
	\[
	\vp_i^k=(0, \alpha_i^k):=\left(0, \left(\frac i{k}-\frac{1}{2k}\right)\left(1-\frac1e\right)\right)
	\]
	and each $\vp_i^k$ has mass:
	\[
	\gvec_k(\vp_i^k):=\int_{\alpha_i^k-\Delta_k}^{\alpha_i^k+\Delta_k}\frac{1}{1-x}dx=\log\left(\frac{1-\alpha_i^k+\Delta_k}{1-\alpha_i^k-\Delta_k}\right).
	\]
	where for convenience we defined $\Delta_k=\frac{1}{2k}\left(1-\frac1e\right)$.
	
	Note that the $\gvec_k$ is a well defined distribution, indeed we have that:
	\begin{align*}
	\sum\limits_{i=1}^k\gvec(\vp_i^k)&=\sum\limits_{i=1}^k\log\left(\frac{1-\alpha_i^k+\Delta_k}{1-\alpha_i^k-\Delta_k}\right)\\
	&=\log\left(\prod\limits_{i=1}^k\frac{1-\alpha_i^k+\Delta_k}{1-\alpha_i^k-\Delta_k}\right)\\
	&=\log\left(\prod\limits_{i=1}^k\frac{1-\alpha_i^k+\Delta_k}{1-\alpha_i^k-\Delta_k}\right)\\
	&=\log\left(\prod\limits_{i=1}^{k-1}\frac{1-\alpha_{i}^k+\Delta_k}{1-\alpha_{i+1}^k+\Delta_k}\frac{1-\alpha_k^k+\Delta_k}{1-\alpha_k^k-\Delta_k}\right)\\
	&=\log\left(\frac{1-\alpha_1^k+\Delta_k}{1-\alpha_k^k-\Delta_k}\right)\\
	&=\log(e)\\&=1.
	\end{align*}
	where we used that by construction that $\alpha_{i+1}^k=\alpha_{i}^k+2\Delta_k$
	Now observe that for the considered instance, any randomized contract $\gvec_k\in\cP^R$ we have that:
	\[
	\OPT(\vc)-U(\gvec_k,\vc)=1-c_a-\sum\limits_{i:a_i^k\ge c_a}\gvec(\vp_i^k)(1-a_i^k).
	\]
	In particular the gap continues to decrease linearly in $c_a$ until a point $a_i^k$ is met, in which the function jumps up by $\gvec(\vp_i^k)(1-a_i^k)$ and for $c_a$ the function starts from $\sum_{i=1}^ka_i^k\gvec_k(\vp_i^k)$.
	
	\begin{align}
		\gvec(\vp_i^k)(1-a_i^k)&=\frac{e(1+2k)-1-2i(e-1)}{2ek}\log\left(1+\frac{e-1}{ek-i(e-1)}\right)\\
		&\ge\frac{e(1+2k)-1-2i(e-1)}{2ek}\frac{e-1}{e(1+k)-1-i(e-1)}\\
		&\ge\frac{(e-1)(1+e(2k-1))}{2e^2k^2}=\Theta(1/k)
	\end{align}
	where we used that $\log(1+x)\ge1-\frac{1}{x+1}$ and that the last function is decreasing and thus its maximum is in $i=1$.
	
	On the other hand
	\begin{align}
		\sum\limits_{i=1}^k\gvec(\vp_i^k)a_i^k&=\sum\limits_{i=1}^k a_i^k\int\limits_{a_i^k-\Delta_k}^{a_i^k+\Delta_k}\frac{1}{1-x}dx\\
		&\le\sum\limits_{i=1}^k \int\limits_{a_i^k-\Delta_k}^{a_i^k+\Delta_k}\frac{x}{1-x}dx\\
		&\le \int\limits_{0}^{1-1/e}\frac{x}{1-x}dx\\
		&=1/e
	\end{align}
	
	On the other hand we can easily prove that for all $i\in[1,\ldots,k]$
	\begin{align}
		\gvec(\vp_i^k)a_i^k&\ge2\frac{a_i^k\Delta_k}{1-a_i^k}\\
		&>\Delta_k\left(\frac{a_i^k-\Delta_k}{1-a_i^k+\Delta_k}+\frac{a_i^k+\Delta_k}{1-a_i^k-\Delta_k}\right)-\xi_k\\
		&\ge \int\limits_{a_i^k-\Delta_k}^{a_i^k+\Delta_k}\frac{x}{1-x}dx-\xi_k
	\end{align}
	where $\xi_k=\frac{(e-1)^3}{2k(k+e-1)(2k+e-1)}=\Theta(1/k^3)$.
	And thus:
	\begin{align}
	\sum\limits_{i=1}^ka_i^k\gamma(\vp_i^k)&>\sum\limits_{i=1}^k\int\limits_{a_i^k-\Delta_k}^{a_i^k+\Delta_k}\frac{x}{1-x}dx-k\xi_k\\
	&=\int\limits_{0}^{1-1/e}\frac{x}{1-x}dx-k\xi_k\\
	&=\frac{1}{e}-k\xi_k\\&=\frac1e-\Theta(1/k^2)
	\end{align}
	This proves that each jump bring the function above $1/e+\Theta(1/k)$.
	Which means that there for all $k$ sufficiently large, there exists a point arbitrary close to some $a_i^k$ for which 
	\[
	\sup\limits_{\vc\in\cC}\OPT(\vc)-U(\gvec_k,\vc)\ge\frac1e+\Theta(1/k).
	\]
	
	\xhdr{Part 2}\ma{citare regret minimizing persuasion}
	On the other hand we can show that all randomized contracts obtain strictly less $1/e$. To prove this part we will use a distribution $\mu\in\Delta(\cC)$ and show that $\mathbb{E}_{\vc\sim\mu}[\OPT(\vc)-U(\gvec,\vc)]=1/e$ for all randomized contracts $\gvec$.
	By using a probabilistic argument we can conclude that only one of the following is true, either $\OPT(\vc)-U(\gvec,\vc)=1/e$ for all $\vc$ or there exists a $\vc^\star(\gvec)$ such that:
	\[
	\OPT(\vc^\star(\gvec))-U(\gvec,\vc^\star(\gvec))<\frac1e.
	\]
	which shows that randomized contract cannot achieve their minimum which is $1/e$.
	
	
	
\end{proof}

\subsection{Existence of optimal menu of deterministic contracts}

First we show that any optimal deterministic menu of contract as size at most $n$.

\begin{lemma}
	The optimal menu has size at most $n$.
\end{lemma}

\begin{proof}
	vedere se esiste già.
\end{proof}

\begin{theorem}
	maximum exists. same proof of before.	
\end{theorem}







\section{Dependence on uncertainty}

Let $\cC\subset[0,1]^{|A|}$ be a convex set, and let $\vc_0\in\cC$ be a ``special'' point in $\cC$ \ma{deve avere la proprietà che sia il centro se $\cC$ è simmetrico. Tipo il baricentro ma anhe altri punti vanno bene.}

Then for all $\delta\in[0,1]$, define $\cC_\delta=\{\delta\vc+\vc_{0}(1-\delta), \forall \vc \in\cC\}=\delta \cC+\vc_0(1-\delta)$. Note that $\vc_0$ is a fixed point of the map $\delta\mapsto\cC_\delta$, and that $\cC_1=\cC$,  $\cC_0=\{\vc_0\}$ and that for all $\delta\in[0,1]$, we have $\cC_\delta \subset \cC$. The parameter $\delta$ measures the ``level'' of uncertainty on the costs vector.

\begin{lemma}
	\[
	\diam(\cC_\delta) = \delta\diam(\cC_1)
	\]
\end{lemma}
Thus 
\[
\inf\limits_{\vp\in\determ}\reg_\delta(\vp) \le\sqrt{\delta}
\]

\begin{theorem}
	Define $f_\delta:=\inf\limits_{p\in\Pi}\sup\limits_{\vc\in\cC_\delta}\reg_\delta(\vp)$.
	Then 
	\[
	f_{\delta+h}-f_\delta\le\sqrt{h}.
	\]
\end{theorem}


\section{Holder continuity is tight in $\delta$}

The following show that the holder exponent is tight. 

\textcolor{red}{capire se dire}Notice that for larger $\delta$ it is true that the gap is constant and hence $O(\delta)$.


\begin{lemma}
	We show that for each $\delta\in [0,1]$, there is an instance such that $f_0-f_\delta\ge \sqrt{\delta}/3$. 
\end{lemma}

\begin{proof}
	
	Build the following instance: There are two actions: $a_1,a_2$. $a_1$ induces outcome $\omega_1$ with probability $1$. On the other hand action $a_2$ induces outcome $\omega_1$ with probability $1-\alpha$ and outcome $\omega_2$ with probability $\alpha$.
	The action $a_2$ costs $c_2=0$ and action $a_1$ has uncertain cost $c_1\in\{0,\delta\}$. Thus $\cC=\{(0,0),(\delta,0)\}$ and $\diam(\cC)=\delta$.
	
	Note that the value of the principal of the first action is $1-p_{\omega_1}$ while the value of the second action is $(1-p_{\omega_1})(1-\alpha)-p_{\omega_2}\alpha$ which is always inferior to the utility of the first action. Moreover if $c_1=0$ and $c_2=0$ then every $p_1\ge p_2$ induces action $a_1$ and if $c_1=\delta$ then any $p_1\ge p_2+\delta/\alpha$. Thus for every contract there exists a contract with $p_2=0$ that dominates it.
	
	Now let's consider two different contracts $\cP_1$ and $\cP_2$, where \[
	\cP_1:=\{\vp=(p_1, 0): p_1\ge\delta/\alpha\}
	\] 
	and 
	\[
	\cP_2:=\{\vp=(p_1, 0): p_1<\delta/\alpha\}
	\] 
	
	Consider the gap function $\vp\mapsto\sup\limits_{\vc\in\cC}[\OPT(\vc)-U(\vp,\vc)]$.
	For all $\vp\in\cP_1$ we have that action $a_1$ is incentivized for all $\vc$ and thus the utility $U(\vp,\vc)$ of the principal is $1-p_1$ for all $\vc\in\cC$. On the other hand for all $\vp\in\cP_2$, we have that if $c_{a_1}=0$ then action $a_1$ is incentivized while if $c_{a_1}=\delta$ we have that action $a_2$ is incentivized. This means that $U(\vp,\vc)=1-p_1$ if $\vc=(0,0)$ and $U(\vp,\vc)=(1-\alpha)p_1$ if $\vc=(\delta,0)$. 
	
	
	
	======================= OLD2 ====================
	
	Note that the value of the principal of the first action is $1-p_{\omega_1}$ while the value of the second action is $(1-p_{\omega_1})(1-\alpha)-p_{\omega_2}\alpha$ which is always inferior to the utility of the first action. Thus the principal need to incentivize the first action.
	
	\xhdr{Case: $c_{1}=0$} Then to incentiveze the first action we require that $p_1\ge p_2$, and $\OPT(\vc)-U(p,c)=1-(1-p_1)=p_1$.
	
	\xhdr{Case $c_1=\delta$} To incentivize action $a_1$ we need:
	\[
	p_1-\delta\ge p_1(1-\alpha)+\alpha p_2
	\]
	which implies that $p_1\ge p_2+\delta/\alpha$. 
	
	The gap also in this case is $\OPT(\vc)-U(p,c)=1-(1-p_1)=p_1$.
	Thus we need to minimize $p_1$ with the constraint $p_1\ge p_2+\delta/\alpha$ which is the contract $p_1=\delta/\alpha$ and $p_2=0$ which gives gap $\delta/\alpha$.
	
	======= OLD =======
	
	Given a $\delta\in (0,1)$, we build an instance with two actions $a_1$ and $a_2$, and two outcomes $\omega_1$ and $\omega_2$. The first action induces outcome $\omega_1$ with probability $1$, while  action $a_2$ induces outcome $1$ with probability $1-2\sqrt{\delta}$ and outcome $\omega_2$ with probability $2\sqrt{\delta}$.
	$\mathcal{C}=[0,\delta]^2$, \emph{i.e.}, both actions has cost in $[0,\delta]$. \textcolor{red}{capire se usare la notazione $\mathcal{C}_\delta$}
	
	We show that that any robust contract is at least $\sqrt{\delta}/3$ suboptimal.
	
	Suppose by contraddiction that there exists a contract that is $\sqrt{\delta}/3$-optimal.
	Since the contract is $\sqrt{\delta}/3$-optimal when $c_{a_1}=c_{a_2}=0$, it holds $p_{\omega_1}\le\sqrt{\delta}/3$.
	%
	Moreover, since the contract is $\sqrt{\delta}/3$-optimal when  $c_{a_1}=\delta$ and $c_{a_2}=0$, it must be the case that the agent is incentivized to play $a_1$. This implies that 
	\[ p_{\omega_1} -\delta\ge  p_{\omega_1} (1-2\sqrt{\delta}) , \]
	and 
	\[p_{\omega_1}\ge \frac{\sqrt{\delta}}{2}. \]
	Hence, we reach a contradiction.
\end{proof}

